Federated Learning with a Single Shared Image

Federated Learning (FL) enables multiple machines to collaboratively train a machine learning model without sharing of private training data. Yet, especially for heterogeneous models, a key bottleneck remains the transfer of knowledge gained from each client model with the server. One popular method, FedDF, uses distillation to tackle this task with the use of a common, shared dataset on which predictions are exchanged. However, in many contexts such a dataset might be difficult to acquire due to privacy and the clients might not allow for storage of a large shared dataset. To this end, in this paper, we introduce a new method that improves this knowledge distillation method to only rely on a single shared image between clients and server. In particular, we propose a novel adaptive dataset pruning algorithm that selects the most informative crops generated from only a single image. With this, we show that federated learning with distillation under a limited shared dataset budget works better by using a single image compared to multiple individual ones. Finally, we extend our approach to allow for training heterogeneous client architectures by incorporating a non-uniform distillation schedule and client-model mirroring on the server side.

==> tables/_app_fedprox_hetero.tex <==
\small
\centering
\begin{tabular}{l|l}
    \toprule
    \multicolumn{1}{c|}{\textbf{FedProx Factor}} & \multicolumn{1}{c}{\textbf{Accuracy}} \\
    \midrule
    0 & 78.67 $\pm$ 0.45 \\
    0.5 & 77.45 $\pm$ 2.24 \\
    1 & 76.47 $\pm$ 3.02 \\
    1.5 & 78.16 $\pm$ 1.72 \\
    2 & \textbf{78.48 $\pm$ 1.12} \\
    \bottomrule
\end{tabular}
\caption{Heterogeneous private data distribution with $\alpha = 1.0$ in Dirichtlet distribution.}
\label{tab:fedprox_factor:hetero}

==> tables/_app_fedprox_homo.tex <==
\small
\centering
\begin{tabular}{l|l}
    \toprule
    \multicolumn{1}{c|}{\textbf{FedProx Factor}} & \multicolumn{1}{c}{\textbf{Accuracy}} \\
    \midrule
    0 & 81.16 $\pm$ 0.53\\
    0.5 & 81.18 $\pm$ 0.42 \\
    1 & 81.92 $\pm$ 0.11\\
    1.5 & 81.4 $\pm$ 0.81\\
    2 & \textbf{81.94 $\pm$ 0.57} \\
    \bottomrule
\end{tabular}
\caption{Homogeneous private data distribution with $\alpha = 100.0$ in Dirichtlet distribuition.}
\label{tab:fedprox_factor:homo}
